Discerning Legitimate Failures From False Alerts: A Study of Chromium's Continuous Integration

Flakiness is a major concern in Software testing. Flaky tests pass and fail for the same version of a program and mislead developers who spend time and resources investigating test failures only to discover that they are false alerts. In practice, the defacto approach to address this concern is to rerun failing tests hoping that they would pass and manifest as false alerts. Nonetheless, completely filtering out false alerts may require a disproportionate number of reruns, and thus incurs important costs both computation and time-wise. As an alternative to reruns, we propose Fair, a novel, lightweight approach that classifies test failures into false alerts and legitimate failures. Fair relies on a classifier and a set of features from the failures and test artefacts. To build and evaluate our machine learning classifier, we use the continuous integration of the Chromium project. In particular, we collect the properties and artefacts of more than 1 million test failures from 2,000 builds. Our results show that Fair can accurately distinguish legitimate failures from false alerts, with an MCC up to 95%. Moreover, by studying different test categories: GUI, integration and unit tests, we show that Fair classifies failures accurately even when the number of failures is limited. Finally, we compare the costs of our approach to reruns and show that Fair could save up to 20 minutes of computation time per build.

==> 7_discussion.tex <==
\section{Discussion}

% Potentially discuss about using \fade and rerun together.
